QuadWBG: Generalizable Quadrupedal Whole-Body Grasping

Legged robots with advanced manipulation capabilities have the potential to significantly improve household duties and urban maintenance. Despite considerable progress in developing robust locomotion and precise manipulation methods, seamlessly integrating these into cohesive whole-body control for real-world applications remains challenging. In this paper, we present a modular framework for robust and generalizable whole-body loco-manipulation controller based on a single arm-mounted camera. By using reinforcement learning (RL), we enable a robust low-level policy for command execution over 5 dimensions (5D) and a grasp-aware high-level policy guided by a novel metric, Generalized Oriented Reachability Map (GORM). The proposed system achieves state-of-the-art one-time grasping accuracy of 89% in the real world, including challenging tasks such as grasping transparent objects. Through extensive simulations and real-world experiments, we demonstrate that our system can effectively manage a large workspace, from floor level to above body height, and perform diverse whole-body loco-manipulation tasks.

==> fig/fig_benchmark.tex <==
\begin{figure}[t]
\centering
% \hspace{-8mm}
\includegraphics[width=0.9\linewidth]{fig/img/energy_vs_performance.png}
\caption{Evaluation of locomotion policies based on AsymAC\cite{pinto2017asymmetric}, ROA\cite{fu2023deep}, StateEstimator\cite{margolis2023walk}, and Teacher-student\cite{hoeller2024anymal} along with baselines.}
% \vspace{-6mm}
\label{fig:locomotion_performance}
\end{figure}

==> fig/fig_dataset.tex <==
\begin{figure}[t]
\centering
\rotatebox{90}{
    \includegraphics[trim={40mm 40mm 30mm 20mm}, clip, width=0.4\linewidth]{fig/img/dataset.png}
}
\caption{Dataset in real world}
\vspace{-6mm}
\label{fig:grasping_fusion}
\end{figure}


==> fig/fig_deployment.tex <==
\begin{figure}[ht]
\centering
\begin{overpic}
[width=0.95\linewidth]
%[width=\linewidth,grid,tics=10]
{fig/img/deployment_v1.png}
    %\put(12,30.5){\footnotesize (a)}
    %\put(38,30.5){\footnotesize (b)}
    %\put(65,30.5){\footnotesize (c)}
    %\put(87.5,30.5){\footnotesize (d)}
\end{overpic}
\caption{From left to right action, mention what is happening.}

\vspace{-0.5cm}
\label{fig:pipeline}
\end{figure}


==> fig/fig_experiment.tex <==
\begin{figure}[t]
\centering
\vspace{2mm}
\begin{overpic}
[width=\linewidth]
%[width=\linewidth,grid,tics=10]
{fig/img/experiment2_v1.png}
    %\put(12,30.5){\footnotesize (a)}
    %\put(38,30.5){\footnotesize (b)}
    %\put(65,30.5){\footnotesize (c)}
    %\put(87.5,30.5){\footnotesize (d)}
\end{overpic}
\caption{
Change this to ours, also mention the table, by adding Tiffany and Deep Wholebody max workspace.
}
\vspace{-6mm}
\label{fig:grasping_fusion}
\end{figure}


==> fig/fig_experiment2.tex <==
\begin{figure}[t]
\centering
\vspace{2mm}
\begin{overpic}
[width=\linewidth]
%[width=\linewidth,grid,tics=10]
{fig/img/experiment2_v1.png}
    %\put(12,30.5){\footnotesize (a)}
    %\put(38,30.5){\footnotesize (b)}
    %\put(65,30.5){\footnotesize (c)}
    %\put(87.5,30.5){\footnotesize (d)}
\end{overpic}
\caption{
Change this to ORM space.
}
\vspace{-6mm}
\label{fig:grasping_fusion}
\end{figure}

